Analyzing Text Representations under Tight Annotation Budgets: Measuring Structural Alignment

Annotating large collections of textual data can be time consuming and expensive. That is why the ability to train models with limited annotation budgets is of great importance. In this context, it has been shown that under tight annotation budgets the choice of data representation is key. The goal of this paper is to better understand why this is so. With this goal in mind, we propose a metric that measures the extent to which a given representation is structurally aligned with a task. We conduct experiments on several text classification datasets testing a variety of models and representations. Using our proposed metric we show that an efficient representation for a task (i.e. one that enables learning from few samples) is a representation that induces a good alignment between latent input structure and class structure.

==> notes.tex <==
%\title{Understanding The Effectiveness of Text Representations Under Tight Annotation Budgets}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Abstract

%Task: Analyze the performance of sequence classifiers with small %annotation budgets. 
%Show that the choice of representation (more than the model) is %critical in these scenarios.
%(not surprisingly, generalization performance depends critically on the %chosen representation.
%We ask why is the representation so critical in low-budget scenarios. %We propose a framework to answer this question (more related to probing %representations) by proposing a metric that measures how good a %representation is aligned to a task, a good representation for a task %is one that results in a good alignment between the latent input %structure and the class structure.
%\newline
%Contributions:
%\begin{itemize}
 %   \item Large scale evaluation across 4 text classification datasets %and three different models of the importance of representation under %low-budget training. Contextual pre-trained word embeddings are %significantly better than baseline sparse representations.
  %  \item Why are pretrained word embeddings critical under low budget %scenarios. We propose a metric to analyze this. Our evaluation metric %is based on structural alignment between input (on the given %representation space) and class structure. The metric shows the %superiority of pre-trained word embeddings over sparse %representations accross a variety of tasks.
   % \item We use the clustered representation for sampling, for %learning under a budget ( similar to cold start)
%\end{itemize}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Related Work

%What is the main difference from prior work? Emphasis on budget learning rather than active learning.
%Our contribution and focus, is more on understanding why good representations are important, they capture the structure on the right way.

%%%
% Related work from testing representations for active learning.
%\paragraph{Testing representations for Active Learning.}

% ore in this line we have the Data-Dependent Complexity developed in \cite{yauney-mimno-2021-comparing}, which measures the strength in patterns of the representation by decomposition of a document similarity matrix and looks at the alignment with task labels. This serves both to compare the quality of representations as well as giving a measure of complexity for classification tasks. Similarly we compare representations, but want to do it specifically in cold-start scenarios. We find different results for BERT-derived representations using \texttt{[CLS]} token.

%Some of these studies focus on feature construction useful for AL, or guiding representation learning using %AL \cite{zhang_active_2017}. In general, the adequateness of newer contextual representation in AL is %acknowledged  and attention is mostly attracted by AL sampling functions. But we %would like to also understand why a representation is appropriate and what choices would work best at first %chance, i.e. in low-budget annotation scenarios.

%\cite{lu_investigating_2019} difference: they show similar results in terms of learning curve; transformers based is better than BOW or ``traditional'' word based embeddings, but they do not do it across different models and do not attempt to explain WHY they might be better for active learning.

%%%
%Related work from probing sentence representations.

% \paragraph{Analysis of sentence representations.}
% After the success of modern contextual text representations, the need for understanding their effectiveness has driven the attention to studying the inner properties of such representations. Many studies focus on testing the behaviour of such models using probing tasks that signal different linguistic capabilities. Building from natural inference probing tasks \cite{conneau-etal-2017-supervised} and other syntactic and semantic abilities \cite{conneau-etal-2018-cram}, SentEval \cite{conneau-kiela-2018-senteval} gathers a full collection of such tasks and provides with an evaluation framework. Paralleling this idea we find other linguistic probe suites \cite{liu-etal-2019-linguistic}, in this case more interested on transfer learning and pointing to the importance of the pre-training task. 
% Language models have been also evaluated for symbolic reasoning \cite{talmor-etal-2020-olmpics}, comparing to learning curves of control models, or tested their ability to distinguish grammatical sentences \cite{marvin-linzen-2018-targeted}. Others have targeted the capacity of this type of representation to transfer linguistic content \cite{ravishankar-etal-2019-probing}.

% The structural aspects of language have been also studied in representations using behavioural analysis. \cite{miaschi-dellorletta-2020-contextual} include probes for dependencies, studying how the contextual capacities of its word representations can be scaled to full sentence embeddings.
% In a similar vein, using linear transformations on the word representations, \cite{hewitt-manning-2019-structural, reif_visualizing_2019} find syntactic structures latent in its vector space.
% In the multi-lingual setting, it has been found structure in the representations, using hierarchical clustering, similar to that of natural language families \cite{singh-etal-2019-bert} that discourage the idea of presence of universal language features.
% Even ontologies have been discovered inside the embeddings, using probing tasks to induce structure as weakly supervised clusters and find hierarchies of latent semantic representations. We follow the idea of finding structure using clusters in the representations, although this work uses a fixed amount of semantic classes as a hyperparameter. The authors consider classical clustering application to be less sensible due to its bias to salient features in the clusters. We believe this problem can be alleviated by using hierarchical clustering at many different granularity levels.

% Departing from behavioural analysis, we now look at approaches that analyze the properties of representations directly, without an intermediate task. Focusing on those that can be used to compare different representations, we have a correlation method called Singular Vector Canonical Correlation Analysis \cite{saphra-lopez-2019-understanding} that have been used to compare representations during consecutive pre-training stages, to study its dynamics, and of different language models. We are also interested in comparing representations, and this type of method is interesting for being independent, but we are more interested in the applicability of representations to particular tasks. More in this line we have the Data-Dependent Complexity developed in \cite{yauney-mimno-2021-comparing}, which measures the strength in patterns of the representation by decomposition of a document similarity matrix and looks at the alignment with task labels. This serves both to compare the quality of representations as well as giving a measure of complexity for classification tasks. Similarly we compare representations, but want to do it specifically in cold-start scenarios. We find different results for BERT-derived representations using \texttt{[CLS]} token.

%\cite{conneau-etal-2017-supervised} Supervised Learning of Universal Sentence Representations from Natural Language Inference Data. Conneau et.al. -downstream task (NLI) evaluation of sentence vectors. 2018, pre-bert world, discuss the usefulness of sentence vectors vs word vectors.
%\cite{conneau-etal-2018-cram} Probing sentence embeddings for *linguistic* properties: Surface, Syntactic,semantic information. Based on LSTMs.
%\cite{conneau-kiela-2018-senteval} SentEval: collection of downstream tasks for evaluation of sentence vectors.
%None of the above focus on low budget annotation.
%\cite{marvin-linzen-2018-targeted}: probing tasks of gramaticality in LMs.
%\cite{miaschi-dellorletta-2020-contextual} linguistic probing tasks, study several layer strategies, compares with GloVe.
%\cite{talmor-etal-2020-olmpics}: Probing MLM tasks for symbolic reasoning. zero-shot evaluation (no fine-tuning), as well as comparing the learning curve of a fine-tuned LM to the learning curve of multiple controls.
%\cite{liu-etal-2019-linguistic}: probing contextual word representations using probing models of several linguistic tasks (semantic, syntactic). transferability in representation layers. choice of pretraining task affect.

%Structure
%\cite{michael-etal-2020-asking}: Asking without Telling: Exploring Latent Ontologies in Contextual Representations. modification to classifier-based probing that induces a latent categorization (or ontology) of the probe’s input.
%\cite{hewitt-manning-2019-structural}: A Structural Probe for Finding Syntax in Word Representations. Linear transformation approach. Focus on syntax: distance between words in the parse tree, and depth in the parse tree. Syntax is implicit in contextual representations.
%\cite{reif_visualizing_2019} Visualizing and Measuring the Geometry of BERT: extension of the previous. focus on syntax. Visualization. 

%Multilingual:
%\cite{ravishankar-etal-2019-probing} focuses on probing-centric evaluations, and their extension to a multilingual domain. This type of evaluation require probing classification models.
%\cite{singh-etal-2019-bert}: BERt is not an interlingua and the Bias of Tokenization. Analysis using hierarchical clustering of multilingual contextual representations. Finds hierarchical similarity relations akin to the language families.

%Descriptive analysis:
%\cite{saphra-lopez-2019-understanding}: (SVCCA) Analysis of deep (LSTM-based) language models inner representation learning and its dynamics by correlation between layer representations of target model and task-specific trained models.
%\cite{kudugunta-etal-2019-investigating}: (SVCCA), a representation similarity framework that allows us to compare representations across different languages, layers and models. 

%\cite{yauney-mimno-2021-comparing}: They also seek alignment with task labels to assess the quality of representations. They don't look at the AL scenario. Theoretical approach, not empirical. For representation comparison they use [CLS]. When they compare different layer strategies, they find no real change between them, we do find differences, at least in the AL scenario.

%%%
%Related work on using clustering for cold start in active learning.
% \paragraph{Cold-start sampling via clustering.}
% The direct use of clustering for setting the initial seeds has been studied at least since \cite{olsson_literature_2009}, but its regarded a not very influential aspect. In the surveys \cite{schroder_survey_2020, aggarwal_active_2014} we find this technique as representational AL methods that don't require a previously labelled subsample. An example of selection of initial text samples using k-means can be found in \cite{kang_using_2004} or with k-medoids for computer vision in \cite{nguyen_active_2004}. Clustering has been used for feature crafting as well, with centroid-distances as features for guiding the selection of batches of documents by topic in \cite{poursabzi-sangdeh-etal-2016-alto} or for cold-start AL of clinical reviews in \cite{hashimoto_topic_2016}. More recently, \cite{shnarch-etal-2022-cluster} recognize the difficulty of using modern contextual representations in cold-start due to its instability. They propose an intermediate phase, previous to fine-tuning, where they try to predict cluster labels.

% \cite{brangbour_active_2020} use the idea of impurity criterion to assess cluster quality. They later use it in a multi-modal scenario with complex label distributions in \cite{brangbour_cold_2022}, where clusters are first ranked by a quality metric. They apply a semi-supervised setting in an attempt to fix the poor alignment of samples with the scarce positive class.

% Previously presented literature is more focused on flat clustering techniques. We agree with the idea that a hierarchical clustering can be helpful in discovering structure in representations \cite{dasgupta_hierarchical_2008}. We think this technique can help to alleviate the problem of sample-class alignment. In general, the effect of cold-start clustering over different representations is largely unexplored.

%\cite{olsson_literature_2009} A literature survey of active machine learning in the context of natural language processing: seed set problem. Claims that  clustering doesn't help much.
%\cite{aggarwal_active_2014} "Active learning: A survey": Representativeness-Based Models. AL that can work without annotated samples.
%\cite{schroder_survey_2020} A survey of AL for text class. using deep NN:
%  - \cite{nguyen_active_2004} Active Learning Using Pre-clustering: method of finding representatives for cold-start using k-medoid clustering. "the goal of clustering is data representation rather than data classification". Experiments in computer vision, doesn't use different representations.
%  - \cite{dasgupta_hierarchical_2008}: Hierarchical clustering for AL.
%  - \cite{poursabzi-sangdeh-etal-2016-alto}: ALTO: Active Learning with Topic Overviews for Speeding Label Induction and Document Labeling. flat clustering to select topics.

%\cite{brangbour_cold_2022} Cold Start Active Learning Strategies in the Context of Imbalanced Classification.: multi-modal scenario, clustering,
%\cite{brangbour_active_2020}: impurity criterion.

%\cite{kang_using_2004} Using Cluster-Based Sampling to Select Initial Training Set for Active Learning in Text Classification
%\cite{zhu-etal-2008-active}: Active Learning with Sampling by Uncertainty and Density for Word Sense Disambiguation and Text Classification: k-means clustering and closest-to-centroid sample representatives. Fixed amount of clusters. Doesn't study the effect of different representations.
%\cite{hashimoto_topic_2016} Topic detection using paragraph vectors to support active learning in systematic reviews: After detecting latent topics in a collection of documents, we represent each document as a k-dimensional feature vector by calculating the distance of the document to the k cluster centroids.

%\cite{shnarch-etal-2022-cluster}: adding an intermediate unsupervised classification task, between the pre-training and fine-tuning phases. As such an intermediate task, we perform clustering and train the pre-trained model on predicting the cluster labels. scarce budget, clustering, BUT focuses on fine-tuning a pre-trained model for improving text classification. considers the importance of intermediate tasks closer to classification that improves the final model, doesn't consider the importance of representations.

%% Need initial seed:
% \cite{xu_representative_2003} Representative sampling for text classification using support vector machines. Needs previous subsamples
%\cite{singh_improving_2018} Improving Active Learning in Systematic Reviews: AL, feature extraction, topic modelling, random first seed.

%% Clustering in AL selection functions:
%\cite{yuan-etal-2020-cold}: ALPS. use clustering of BERT embeddings to choose samples in AL, slightly different from low-budget learning.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Datasets and Text Representations

%\subsection{Datasets and Text Representations}

% IMDB
% 25K / 25K train 25k, test 25k, unsup. 50k \\
% WT
% 202165, 21384 & train 159571, test 63978 \\
% CC 
% 1839732, 159782 & train 1,804,874, dev 97,320, test 97,320 \\
% s140
% 800177, 800182 & train 1.6M, test 498 \\

%\textbf{IMDB} \cite{maas-etal-2011-learning} is a sentiment binary classification dataset. It consists of a series of movie reviews from the famous film enthusiasts website of the same name, where the task is to predict the sentiment, positive or negative, of those reviews. Complementary to the supervised task, it includes an unsupervised partition, that we can use to enrich some of the representations.

%The other balanced distributed dataset is sentiment140 or \textbf{s140} \cite{go_twitter_2009}. It consists of a collection of messages of the micro-blogging platform Twitter. The task consist of predicting the mood of the comments, whether positive or negative.

%As unbalanced dataset we first have \textbf{WikiToxic} \cite{wulczyn_ex_2017}. It consists of user discussion comments of editors of the Wikipedia website. Comments are labeled by persons considering for toxic behaviour, that is, for abuse, harassment, or other forms of non-constructive language. For our experiments we have applied a cleaning algorithm that removes any non-alphanumeric character and HTML markup.

%The fourth option considered \textbf{CivilComments} \cite{borkan_nuanced_2019} dataset, from an archive of the Civil Comments platform, a user comments plugin for news websites. The documents have been tagged buy annotators indicating the presence of toxic language comprising obscene or sexually explicit language, threat, insult or direct attack to other users. This target class is small and the length of the texts tend to be larger than those in WikiToxic. We have also applied the same cleaning process.

% For each of these datasets we have produced representations using a series of models ranging from classical methods to modern contextual representations.
% We use a term frequency bag-of-words (BOW) as baseline for simple representation methods.
% \href{https://nlp.stanford.edu/projects/glove/}{GloVe} \cite{pennington_glove_2014} word vectors pre-trained on Common Crawl (840B cased) and average pooled to get sentence vectors.
% \href{https://fasttext.cc/docs/en/pretrained-vectors.html}{fastText} word vectors (FastT) pre-trained on Wikipedia with average pooling. BERT \cite{devlin-etal-2019-bert} embeddings from BERT-base uncased, 2\textsuperscript{nd} to last layer, producing two sentence representations: average pooling of all tokens (BERTa) and single \texttt{[CLS]} token (BERTc).

%The tokenization process employs a WordPiece tokenizer. First described in \cite{schuster_japanese_2012} and popularized by BERT \cite{devlin-etal-2019-bert}, is a subword-based tokenization algorithm. Employing this method we are able to keep the size of vocabulary small while not needing to remove too frequent or infrequent tokens.

%\paragraph{TF-IDF.}

%\paragraph{SVD.}

%\paragraph{GloVe}
%GloVe \cite{pennington_glove_2014} provides with word embeddings pre-trained on big corpora. It stands for Global Vectors, as it is constructed from the global co-occurrence matrix of the terms in the corpus. It also combines the word-word statistics with a window-based method that encodes the context of words. The objective function is a linear regression defined over the product of these two types of vectors.

%The authors have made public several pre-trained GloVe models\footnote{\url{https://nlp.stanford.edu/projects/glove/}} \footnote{\url{https://github.com/stanfordnlp/GloVe}}. For our experiments, we have employed the models pre-trained on the Common Crawl corpus (a massive text corpus crawled from the Internet): the 840 billion cased tokens version and the 42 billion uncased. Both tokenized using the Stanford tokenizer. From the 300 dimension word vectors obtained, we have applied an average pooling strategy to obtain document vectors.

%\paragraph{fastText}
%This is a word embedding representation method based on word2vec type of models. fastText \cite{bojanowski_enriching_2017, joulin_bag_2016} leverages the use of subword information on top of continuous word vectors. Subword information is encoded as bags of character n-grams. A skipgram model is applied on these bags. Then the vectors obtained are summed to produce word vectors. This methodology helps in representing compounds in words, as well as mitigating the out-of-vocabulary issue.
%
%Several pre-trained models have been published by the authors\footnote{\url{https://fasttext.cc/docs/en/pretrained-vectors.html}}. In this research we have used the word embeddings trained on Wikipedia corpus. The document vectors are obtained using an average pooling strategy over the 300 dimensional fastText word vectors.

%\paragraph{BERT embeddings} \cite{devlin-etal-2019-bert} is a transformer-based model that has shown to improve greatly the performance of NLP models on different benchmarks. It leverages the use of big corpora by pre-training in an unsupervised fashion, and can be later fine-tuned to downstream, more specialised tasks. For this work, we have employed BERT-base (uncased) using HuggingFace Transformers \cite{wolf_transformers_2020} implementation.
%By design, this model also can be used to generate embeddings. The authors experimented with different forms of layer pooling strategies and tested them on downstream tasks. For our experiments we have selected: average of the 12 layers, concatenation of the last 4 and the second to last layer. We take special attention to the latest as being reported by the authors as the most robust between tasks.
%
%At the token level, BERT design includes a special \texttt{[CLS]} token used as an overall document representation. It has been discussed its appropriateness in comparison to other document-level options\footnote{\url{https://github.com/google-research/bert/issues/164\#issuecomment-441324222}}. For comparison, we have created document embeddings with two strategies: a \texttt{[CLS]} token representation and the average pooling of all tokens.


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% SAM

% The metric proposed in this work measures the quality of a representation by looking at the structure of the spatial distribution of labels induced by the representation at test. Each text representation produces a particular organization of the sample labels. We will argue that good representations are those that exhibit structural alignment between this distribution and the distribution of the label classes. 

% In general terms, the method proposed is comprised by an unsupervised methodology, a supervised one, and a bridge between those two realms. In a first phase we employ unsupervised learning strategies to uncover the structure of samples. Then we look at the labels of those samples and analyze them. The device in between by which we connect with the supervised world employs the notion of cluster purity. That is, whether a cluster can separate properly samples by their label classes at a certain level of granularity. We then use this notion to yield label classes per cluster with an associated probability. This gives us a labelling of all the samples considered that we can use to compute the usual supervised metrics, such as accuracy, F1-score or AUC.

%[EXPLANATION OF THE DENDOGRAM FIGURE, IT IS IMPORTANT TO EXPLAIN %HOW EACH LEVEL CORRESPONDS TO A PARTITION WITH K CLUSTERS WHERE k %RANGES FROM N (AT THE BOTTOM) TO 1 (AT THE TOP)] THIS CAN BE %EXPLAINED IN THE CAPTION OF THE DENDOGRAM

% For the unsupervised phase we employ clustering methods to find out structure in the samples. At this step, we don't simply want to use an arbitrary number of clusters. Samples can be disposed in organizations more complex than a bunch of disjoint groups, they can be hierarchical, etc. Choosing a fixed amount of clusters would only allow for the discovery of shallow alignments between the sample structure and label class structure. For this reason we want to compute clusters for all the possible levels of granularity. That is, we allow $k$ to range between $1$ and the total number of samples. This enables clustering methods to uncover more subtle structure in the samples.

% In order to generate clusters for all $k$ we use a hierarchical agglomerative clustering algorithm. This is a bottom-up method that builds up a tree of nested clusters starting from the samples as singleton clusters, merging them according to a similarity metric. We employ Ward's method for merging, which starts with the squared Euclidean distance between samples and then minimizes the total within-cluster variance by finding consecutive pairs of clusters with the minimal increase.

% After the clustering full tree have been computed, we traverse it generating a clustering for each $k$. In this manner, we are able to create all possible levels of granularity without computing a full clustering for each step.
% For efficiency, in our experiments we take i.i.d. samples of size 10k for each dataset and average the results over 5 seeds.

% The \textbf{purity} of a cluster measures the amount of samples with a single label class. A pure cluster would have all samples labelled with the same class. Similarly, a random draw of samples will have, on average, a purity equal to thehttps://www.overleaf.com/project/62949cf0003767076cc80052 most frequent label in the prior distribution. This metric is computed by counting the occurrences of each class, taking the maximum, and weighting by the cluster size:
% $$ pur(C) = \frac{1}{|C|} max(\#(l=l_1), \ldots, \#(l=l_{|L|})) $$

% We also define the \textbf{majority} of a cluster as the label class with the most occurrences:
% $$ maj(C) = arg\,max(\#(l=l_1), \ldots, \#(l=l_{|L|})) $$

% \subsection{Clustering as a classifier}

% We are now able to use the clustering as a classifier. For each cluster we take its majority label as the prediction for all its samples, and its purity as the probability of such prediction. For example, in a cluster with 4 out of 5 positive labels, all samples will be predicted as positive with probability $4/5$. Applying this to all clusters gives us a full dataset prediction with an associated probability.

% In order to measure the level of alignment between a clustering and the underlying label classes, we employ a classification metric on the predictions made by the clustering-as-a-classifier method described before.

% Having class predictions and probabilities for the dataset, we can calculate the common classification metrics used in binary classification, such as accuracy or F-score. In this work we focus on the Area Under the precision-recall curve (AUC), an aggregate metric throughout all possible probability thresholds. This measure portraits the property of threshold-invariability, which is interesting for our purposes as where we are working with both balanced and unbalanced datasets.

%\subsection{Alignment Curves}

% Having a metric of the performance of the predictions made by a given clustering and having a clustering for each number of clusters traversing the agglomerative merging tree, we can extend the classification metric to a function on the number of clusters $k$. This produces a characteristic curve for each representation that we call the Structural Alignment Metric (SAM).

% A clustering with all samples as singleton clusters, is completely pure and exhibits a trivial perfect alignment with the label classes. In the other extreme, a single cluster is maximally mixed and has no alignment. Good representations will move quickly to high levels of alignment as the number of clusters increases.

% The values of this type of curve range from the performance of a classifier that uniformly predicts the majority class when $k=1$ to the performance of a perfect classifier when $k$ is equal to the number of samples, i.e. $1$.

% In order to compare the quality of different representations with a single value, we calculate the area under the SAM curve.

% Because the information portrayed by the values of the curve decreases with the number of clusters increase, as they become trivial, we will focus on the beginning of the curve, up to 1000 samples, in order to compare the representations.


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Experimental Setup

%\subsection{Measuring SAM}
%This section presents the results on measuring SAM over each dataset. Should also include the unsupervised metric for the ones that we have.

%We have computed SAM for all the datasets and text representations just %presented. A summary of the results thus obtained can be found in Table %\ref{tab:sam}. For performance, we took five random sub-samples of 10K examples %for each dataset and averaged the results.
%[The results for the alignment curves and SAM are computed using the first 1000 %points. The relevant information is contained in the first part of the curve, as %the alignment becomes progressively trivial as the number of cluster increases.]

% \subsubsection{Maximum Entropy Model}

% The binary classifier models the probability $P(l|r(x),\theta)$ of a point $x$ belongs to a class $l \in L$, given the representation of the point $r(x)$ and the model parameters $w$:

% \begin{equation}
%     P(l|r(x),w) = \sigma (s)^{l} (1-\sigma(s))^{1-l},
% \end{equation}

% where $l \in \{0,1\}$, $\sum_{l\in\{0,1\}}{P(l|r(x),\theta)} = 1$, $s=w^Tr(x)$, and $\sigma(s) = \frac{1}{1+ \exp^{-s}}$. 

% For each $<r(x),l(x)>$ training tuples, we optimize the following loss $\mathcal{L}$ to learn the model parameters $w$:

% \begin{align}
%     \mathcal{L}(r(x),l(x); w) &= - \log (P(l(x)| r(x), w)) \\
%     &= log(1+\exp^{s}) - l(x)s
% \end{align}        

% Correlation

%To find the correlation between SAM and actual classification performance, we %trained simple binary Maximum Entropy (MaxEnt) classifiers on the same datasets %and representations. We measure the performance starting from 100 up to 1000 %samples giving us the Learning Curves obtained in Figure \ref{fig:lc}. In our %study case, we are interested in the performance of classifiers for different %sizes of the initial pool of labelled examples, not the relative performance of a %particular AL retrieval function. In Table \ref{tab:lc} are the results for the %Area Under the Learning Curve.




% MUST CLARIFY SOMEWHERE THAT IS LEARNING UNDER A BUDGET FROM A RANDOM SAMPLE, I.E. WE ARE LOOKING AT THE 
% STANDARD LEARNING CURVE PERFORMANCE MAYBE THIS CAN BE CLARIFIED IN THE RELATED WORK SECTION

